Feasibility Study for a Next-Generation Mu2e Experiment

We explore the feasibility of a next-generation Mu2e experiment that uses Project-X beams to achieve a sensitivity approximately a factor ten better than the currently planned Mu2e facility.

==> wp-authors_copy.tex <==

%%%\author{Author Names\\
%%%  \textit{\small Their Affiliation}
%%%}

\author{K.~Knoepfel}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{V.~Pronskikh}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{R.~Bernstein}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{R.~Coleman}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{D.~Glenzinski}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{M.~Lamm}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{N.~Mokhov}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{A.~Mukherjee}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{V.~Nagaslaev}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{T.~Page}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{R.E.~Ray}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{V.L.~Rusu}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{R.~Wagner}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
\author{S.~Werkema}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA}
%
%
%
\author{J.~Miller}
\affiliation{Boston University, Boston, Massachusetts 02215, USA}
%
%
%
\author{D.G.~Hitlin}
\affiliation{California Institute of Technology, Pasadena, California 91125, USA}
%
%
%
\author{S.~Miscetti}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
%
%
%
\author{D.N.~Brown}
\affiliation{Lawrence Berkeley National Laboratory and University of California, Berkeley, California 94720, USA}
%
%
%
\author{D.~Hedin}
\affiliation{Northern Illinois University, DeKalb, Illinois 60115, USA}
%
%
%
\author{C.E.~Dukes}
\affiliation{University of Virginia, Charlottesville, Virginia 22906, USA}
%
\author{R.~Ehrlich}
\affiliation{University of Virginia, Charlottesville, Virginia 22906, USA}
%
\author{M.J.~Frank}
\affiliation{University of Virginia, Charlottesville, Virginia 22906, USA}
%
\author{R.C.~Group\footnote{With a Joint Appointment at Fermi National Accelerator Laboratory, Batavia, Illinois 60510, USA.}}
\affiliation{University of Virginia, Charlottesville, Virginia 22906, USA}
%
\author{Y.~Oksuzian}
\affiliation{University of Virginia, Charlottesville, Virginia 22906, USA}


